Preliminary Evidence for Lensing-Induced Alignments of High-Redshift Galaxies in JWST-CEERS

The majority of low-mass ($\log_{10} M_*/M_{\odot}=9-10$) galaxies at high redshift ($z>1$) appear elongated in projection. We use JWST-CEERS observations to explore the role of gravitational lensing in this puzzle. The typical galaxy-galaxy lensing shear $\gamma\sim1\%$ is too low to explain the predominance of elongated early galaxies with ellipticity $e\approx0.6$. However, non-parametric quantile regression with Bayesian Additive Regression Trees reveals hints of an excess of tangentially-aligned source-lens pairs with $\gamma>10\%$. On larger scales, we also find evidence for weak lensing shear. We rule out the null hypothesis of randomly oriented galaxies at $\gtrsim99\%$ significance in multiple NIRCam chips, modules and pointings. The number of such regions is small and attributable to chance, but coherent alignment patterns suggest otherwise. On the chip scale, the average complex ellipticity $\langle e\rangle\sim10\%$ is non-negligible and beyond the level of our PSF uncertainties. The shear variance $\langle\overline{\gamma}^2\rangle\sim10^{-3}$ is an order of magnitude above the conventional weak lensing regime but is more sensitive to PSF systematics, intrinsic alignments, cosmic variance and other biases. Taking it as an upper limit, the maximum implied ``cosmic shear'' is only a few percent and cannot explain the elongated shapes of early galaxies. The alignments themselves may arise from lensing by a protocluster or filament at $z\sim0.75$ where we find an overabundance of massive lens galaxies. We recommend a weak lensing search for overdensities in ``blank'' deep fields with JWST and the Roman Space Telescope.

==> referee_v10_lensing_table_errorprop.tex <==
\begin{table}
\begin{tabular}{cccccccccccccccccccc}
Source ID & Source RA & Source Dec & Source $z$ & Source $\log_{10} (M_*/M_{\odot})$ & Source $R_{\rm e}$ & Source $e$ & Source $\phi$ & Rest Filter & $\theta$ & $\theta_{\rm E}$ & $\gamma$ & $\psi$ & Lens ID & Lens RA & Lens Dec & Lens $z$ & Lens $\log M_*/M_{\odot}$ & Lens $R_{\rm e}$ & Lens $\sigma_*$ \\
23392 & 214.80777 & 52.86992 & $2.619\pm0.044$ & $9.07\pm0.03$ & $1.39\pm0.10$ & $0.673\pm0.020$ & $-69.171\pm2.636$ & F200W & $3.643$ & $2.249\pm0.206$ & $0.309\pm0.028$ & $83.628\pm2.636$ & 23335 & 214.80843 & 52.87069 & $0.823\pm0.023$ & $10.94\pm0.01$ & $2.528\pm0.194$ & $387.05\pm16.47$ \\
24257 & 214.8167 & 52.86969 & $1.118\pm0.061$ & $9.43\pm0.05$ & $1.90\pm0.17$ & $0.142\pm0.028$ & $78.415\pm3.154$ & F115W & $2.605$ & $1.323\pm0.320$ & $0.254\pm0.061$ & $84.312\pm3.154$ & 25049 & 214.81657 & 52.8704 & $0.840\pm0.029$ & $11.27\pm0.03$ & $3.310\pm0.330$ & $492.55\pm28.20$ \\
24459 & 214.81947 & 52.87288 & $2.338\pm0.023$ & $11.23\pm0.01$ & $6.67\pm1.01$ & $0.397\pm0.016$ & $-43.107\pm1.603$ & F200W & $13.734$ & $3.408\pm0.423$ & $0.124\pm0.015$ & $78.321\pm1.603$ & 25049 & 214.81657 & 52.8704 & $0.840\pm0.029$ & $11.27\pm0.03$ & $3.310\pm0.330$ & $492.59\pm28.89$ \\
24638 & 214.83818 & 52.88739 & $2.359\pm0.029$ & $10.89\pm0.07$ & $1.14\pm0.03$ & $0.377\pm0.008$ & $-64.522\pm0.402$ & F200W & $16.117$ & $3.351\pm0.509$ & $0.104\pm0.016$ & $80.828\pm0.402$ & 12631 & 214.84013 & 52.89141 & $0.780\pm0.015$ & $11.12\pm0.01$ & $2.534\pm0.356$ & $473.64\pm35.12$ \\
28283 & 214.85403 & 52.87866 & $3.382\pm0.049$ & $9.45\pm0.01$ & $1.60\pm0.12$ & $0.811\pm0.018$ & $-48.633\pm2.200$ & F356W & $10.399$ & $3.150\pm0.312$ & $0.151\pm0.015$ & $84.810\pm2.200$ & 28072 & 214.85181 & 52.87682 & $0.817\pm0.020$ & $10.75\pm0.03$ & $1.279\pm0.083$ & $435.19\pm20.87$ \\
29037 & 214.85188 & 52.87375 & $2.349\pm0.133$ & $9.06\pm0.06$ & $1.04\pm0.17$ & $0.583\pm0.024$ & $81.108\pm5.014$ & F200W & $11.072$ & $2.728\pm0.286$ & $0.123\pm0.013$ & $81.966\pm5.014$ & 28072 & 214.85181 & 52.87682 & $0.817\pm0.020$ & $10.75\pm0.03$ & $1.279\pm0.083$ & $436.10\pm21.40$ \\
51412 & 214.98434 & 52.89845 & $1.805\pm0.052$ & $10.23\pm0.11$ & $3.30\pm0.22$ & $0.494\pm0.016$ & $34.954\pm1.771$ & F150W & $4.736$ & $1.881\pm0.166$ & $0.199\pm0.018$ & $80.206\pm1.771$ & 51197 & 214.98547 & 52.89777 & $0.719\pm0.009$ & $10.99\pm0.01$ & $3.072\pm0.247$ & $370.27\pm15.64$ \\
54273 & 214.81218 & 52.81713 & $5.119\pm0.052$ & $9.43\pm0.02$ & $1.31\pm0.14$ & $0.522\pm0.030$ & $43.650\pm2.122$ & F356W & $14.683$ & $5.515\pm1.179$ & $0.188\pm0.040$ & $89.716\pm2.122$ & 53095 & 214.80865 & 52.81919 & $0.820\pm0.024$ & $11.24\pm0.01$ & $2.588\pm0.490$ & $545.67\pm55.79$ \\
65925 & 215.1386 & 52.98904 & $2.311\pm0.014$ & $9.22\pm0.02$ & $0.70\pm0.05$ & $0.508\pm0.019$ & $61.166\pm2.291$ & F200W & $5.695$ & $1.470\pm0.129$ & $0.129\pm0.011$ & $79.061\pm2.291$ & 66073 & 215.13988 & 52.98812 & $0.689\pm0.015$ & $10.93\pm0.02$ & $4.039\pm0.289$ & $302.59\pm12.81$ \\
70412 & 215.09525 & 52.93305 & $1.995\pm0.032$ & $10.06\pm0.03$ & $2.21\pm0.20$ & $0.613\pm0.011$ & $-67.699\pm1.035$ & F150W & $2.990$ & $1.708\pm0.135$ & $0.286\pm0.023$ & $80.356\pm1.035$ & 70465 & 215.09496 & 52.93227 & $0.720\pm0.017$ & $10.91\pm0.02$ & $2.983\pm0.190$ & $342.92\pm12.80$ \\
86621 & 214.86714 & 52.79953 & $2.121\pm0.041$ & $9.47\pm0.03$ & $5.90\pm1.26$ & $0.718\pm0.022$ & $60.037\pm5.622$ & F200W & $3.746$ & $4.779\pm0.329$ & $0.638\pm0.044$ & $88.000\pm5.622$ & 86622 & 214.86783 & 52.79875 & $0.800\pm0.020$ & $11.28\pm0.01$ & $2.352\pm0.134$ & $589.05\pm18.28$ \\
86695 & 214.87056 & 52.80254 & $4.764\pm0.067$ & $9.49\pm0.07$ & $1.61\pm0.15$ & $0.248\pm0.018$ & $-53.020\pm2.234$ & F356W & $16.823$ & $6.347\pm0.406$ & $0.189\pm0.012$ & $76.554\pm2.234$ & 86622 & 214.86783 & 52.79875 & $0.800\pm0.020$ & $11.28\pm0.01$ & $2.352\pm0.134$ & $589.09\pm17.98$ \\
87402 & 214.87488 & 52.80144 & $2.850\pm0.094$ & $10.27\pm0.06$ & $2.43\pm0.20$ & $0.371\pm0.020$ & $-28.896\pm1.915$ & F200W & $27.162$ & $5.488\pm0.367$ & $0.101\pm0.007$ & $86.647\pm1.915$ & 86622 & 214.86783 & 52.79875 & $0.800\pm0.020$ & $11.28\pm0.01$ & $2.352\pm0.134$ & $588.60\pm18.22$ \\
94812 & 214.84508 & 52.79176 & $4.247\pm0.146$ & $9.70\pm0.07$ & $1.60\pm0.18$ & $0.606\pm0.028$ & $29.231\pm3.247$ & F356W & $10.169$ & $2.741\pm0.403$ & $0.135\pm0.020$ & $87.646\pm3.247$ & 94939 & 214.84778 & 52.79094 & $0.712\pm0.013$ & $11.07\pm0.02$ & $3.538\pm0.440$ & $380.89\pm27.33$ \\
95439 & 214.86063 & 52.80203 & $1.654\pm0.078$ & $9.07\pm0.04$ & $1.91\pm0.75$ & $0.749\pm0.069$ & $7.401\pm22.201$ & F150W & $5.748$ & $1.396\pm0.147$ & $0.121\pm0.013$ & $87.037\pm22.201$ & 85548 & 214.86221 & 52.80185 & $0.560\pm0.019$ & $10.98\pm0.03$ & $4.727\pm0.314$ & $296.80\pm14.25$ \\
95498 & 214.84607 & 52.78814 & $2.622\pm0.145$ & $9.59\pm0.03$ & $1.11\pm0.11$ & $0.635\pm0.013$ & $-73.424\pm1.987$ & F200W & $11.786$ & $2.402\pm0.343$ & $0.102\pm0.015$ & $86.267\pm1.987$ & 94939 & 214.84778 & 52.79094 & $0.712\pm0.013$ & $11.07\pm0.02$ & $3.538\pm0.440$ & $380.60\pm26.35$ \\
95846 & 214.86427 & 52.79873 & $1.316\pm0.066$ & $10.66\pm0.05$ & $3.49\pm0.19$ & $0.361\pm0.007$ & $-4.828\pm0.416$ & F115W & $12.799$ & $3.026\pm0.344$ & $0.118\pm0.013$ & $85.681\pm0.416$ & 86622 & 214.86783 & 52.79875 & $0.800\pm0.020$ & $11.28\pm0.01$ & $2.352\pm0.134$ & $588.07\pm18.57$ \\
\end{tabular}
\end{table}


==> shear_table_errorprop.tex <==
\begin{table}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccc}
Region & RA & Dec & $N^{\rm all}$ & $p^{\rm all}$ & $\langle e\rangle^{\rm all}$ & $\sigma_{\langle e \rangle}^{\rm all}$ & $\langle \phi\rangle^{\rm all}$ & $\sigma_{\langle \phi \rangle}^{\rm all}$ & $|\overline{\gamma}^2|$ & $\sigma_{|\overline{\gamma}^2|}$ & $|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|$ (F115W) & $\sigma_{|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|}$ (F115W) & $|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|$ (F150W) & $\sigma_{|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|}$ (F150W) & $|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|$ (F200W) & $\sigma_{|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|}$ (F200W) & $|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|$ (F277W) & $\sigma_{|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|}$ (F277W) & $|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|$ (F356W) & $\sigma_{|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|}$ (F356W) & $|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|$ (F444W) & $\sigma_{|e_{\rm gal}\star e_{\rm star}^*|/|\overline{\gamma}^2|}$ (F444W) & $N^{\rm high}$ & $p^{\rm high}$ & $\langle e\rangle^{\rm high}$ & $\sigma_{\langle e \rangle}^{\rm high}$ & $\langle \phi\rangle^{\rm high}$ & $\sigma_{\langle \phi \rangle}^{\rm high}$ & $N^{\rm low}$ & $p^{\rm low}$ & $\langle e\rangle^{\rm low}$ & $\sigma_{\langle e \rangle}^{\rm low}$ & $\langle \phi\rangle^{\rm low}$ & $\sigma_{\langle \phi \rangle}^{\rm low}$ & $N^{\rm early}$ & $p^{\rm early}$ & $\langle e\rangle^{\rm early}$ & $\sigma_{\langle e \rangle}^{\rm early}$ & $\langle \phi\rangle^{\rm early}$ & $\sigma_{\langle \phi \rangle}^{\rm early}$ \\
Survey & nan & nan & 3848 & 0.351439 & 0.008596 & 0.000890 & -76.610408 & 2.856324 & 0.000028 & 0.000008 & 8.043397 & 5.160689 & 12.710213 & 20.741997 & 1.447363 & 0.145500 & nan & nan & 0.113110 & 0.043878 & 0.209793 & 0.250711 & 775 & 0.570323 & 0.012061 & 0.001081 & -7.905382 & 18.127117 & 3073 & 0.155804 & 0.013254 & 0.001070 & -80.664259 & 2.349163 & 1795 & 0.119113 & 0.018636 & 0.001606 & -80.197183 & 2.519887 \\
P1 & 214.984415 & 52.978435 & 452 & 0.066638 & 0.038976 & 0.003063 & -77.855550 & 2.039165 & 0.000576 & 0.000111 & 0.713375 & 0.127404 & 1.300976 & 0.511941 & 1.669166 & 0.447083 & nan & nan & 0.377712 & 0.134202 & 0.021795 & 0.025889 & 107 & 0.811519 & 0.020198 & 0.003630 & 35.733432 & 5.491714 & 345 & 0.018187 & 0.055699 & 0.003794 & -75.537673 & 1.768715 & 197 & 0.011739 & 0.078205 & 0.005788 & -78.680048 & 1.986709 \\
P1\_A & 214.958701 & 52.960792 & 199 & 0.720549 & 0.020503 & 0.004996 & -79.233521 & 6.838656 & 0.000463 & 0.000106 & 0.416439 & 0.068519 & 0.345581 & 0.062749 & 0.747991 & 0.244528 & nan & nan & 0.222084 & 0.161397 & 0.008705 & 0.013571 & 45 & 0.404944 & 0.061930 & 0.008421 & 11.149241 & 2.857883 & 154 & 0.329425 & 0.044365 & 0.006326 & -78.793416 & 3.526933 & 87 & 0.519956 & 0.045370 & 0.009522 & 86.437777 & 5.946934 \\
P1\_B & 215.010129 & 52.996078 & 253 & 0.053044 & 0.054112 & 0.003427 & -77.571261 & 1.917349 & 0.001001 & 0.000183 & 0.665421 & 0.184730 & 0.654481 & 0.156672 & 2.632380 & 0.960431 & nan & nan & 0.333909 & 0.046468 & 0.030292 & 0.028515 & 62 & 0.710748 & 0.034994 & 0.003156 & 76.496916 & 3.507433 & 191 & 0.044051 & 0.065597 & 0.004449 & -73.718189 & 1.987758 & 110 & 0.006606 & 0.110732 & 0.006505 & -74.277122 & 1.891703 \\
P1\_A1 & 214.940923 & 52.960792 & 36 & 0.065806 & 0.124969 & 0.009176 & 87.494525 & 2.213625 & 0.005178 & 0.001155 & nan & nan & 0.265532 & 0.080122 & nan & nan & nan & nan & nan & nan & nan & nan & 6 & 0.779766 & 0.095256 & 0.009270 & 86.258837 & 1.705034 & 30 & 0.091796 & 0.130565 & 0.011323 & 87.699022 & 2.510775 & 20 & 0.216999 & 0.137867 & 0.013514 & 75.118497 & 3.730038 \\
P1\_A2 & 214.958701 & 52.943014 & 49 & 0.813965 & 0.030689 & 0.009761 & -88.482837 & 83.918228 & 0.003371 & 0.000461 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 11 & 0.834455 & 0.043956 & 0.010735 & 32.955434 & 24.931351 & 38 & 0.831499 & 0.035383 & 0.010172 & -30.399747 & 53.268087 & 20 & 0.824904 & 0.052349 & 0.015531 & 62.230160 & 12.375861 \\
P1\_A3 & 214.958701 & 52.978570 & 53 & 0.463524 & 0.062890 & 0.013377 & -50.235209 & 5.957865 & 0.001892 & 0.000484 & 0.533952 & 0.141520 & 0.256174 & 0.247743 & nan & nan & nan & nan & nan & nan & nan & nan & 11 & 0.635722 & 0.101285 & 0.026594 & 15.370043 & 38.399175 & 42 & 0.275632 & 0.093018 & 0.016293 & -57.897640 & 4.010342 & 25 & 0.562865 & 0.076129 & 0.022612 & -58.539075 & 7.917899 \\
P1\_A4 & 214.976479 & 52.960792 & 59 & 0.745130 & 0.037742 & 0.007163 & 40.715718 & 6.197549 & 0.001791 & 0.000253 & nan & nan & nan & nan & nan & nan & nan & nan & 0.072824 & 0.109746 & nan & nan & 15 & 0.091334 & 0.165218 & 0.004144 & 14.388890 & 0.928322 & 44 & 0.728559 & 0.048309 & 0.009981 & 76.167184 & 6.054066 & 22 & 0.978232 & 0.018321 & 0.009432 & -85.628564 & 49.873509 \\
P1\_B1 & 215.027907 & 52.996078 & 55 & 0.789574 & 0.033816 & 0.006385 & 63.395963 & 5.274432 & 0.002319 & 0.000467 & nan & nan & 0.251159 & 0.067884 & nan & nan & nan & nan & nan & nan & nan & nan & 11 & 0.777272 & 0.075589 & 0.011115 & 22.986560 & 4.294749 & 44 & 0.740338 & 0.043270 & 0.007427 & 76.652878 & 4.464896 & 29 & 0.532403 & 0.074580 & 0.009393 & -87.405875 & 3.675142 \\
P1\_B2 & 215.010129 & 53.013855 & 72 & 0.012604 & 0.126447 & 0.006647 & -86.157509 & 1.728347 & 0.006335 & 0.000842 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 21 & 0.708960 & 0.061587 & 0.007125 & -74.336807 & 2.558862 & 51 & 0.011934 & 0.155391 & 0.008634 & -88.045153 & 2.046658 & 29 & 0.011291 & 0.216250 & 0.012556 & -80.694789 & 2.350424 \\
P1\_B3 & 215.010129 & 52.978300 & 65 & 0.554271 & 0.045283 & 0.006255 & -53.782783 & 4.040578 & 0.000801 & 0.000217 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 15 & 0.396438 & 0.114893 & 0.007120 & 70.713987 & 2.395909 & 50 & 0.269088 & 0.077778 & 0.006631 & -41.594116 & 3.234060 & 25 & 0.512342 & 0.079918 & 0.015907 & 89.090154 & 4.249519 \\
P1\_B4 & 214.992352 & 52.996078 & 61 & 0.446611 & 0.058902 & 0.006334 & -56.827203 & 4.277418 & 0.002057 & 0.000534 & 1.883084 & 0.523453 & 0.408427 & 0.128272 & 0.317442 & 0.073679 & nan & nan & 0.165870 & 0.021735 & nan & nan & 15 & 0.996578 & 0.007326 & 0.004116 & -81.967539 & 40.848447 & 46 & 0.372057 & 0.077065 & 0.008284 & -56.517469 & 4.069297 & 27 & 0.094108 & 0.157989 & 0.013167 & -47.372996 & 2.736675 \\
P2 & 214.894881 & 52.915111 & 414 & 0.571282 & 0.019112 & 0.002562 & -46.210442 & 3.852375 & 0.000175 & 0.000046 & 0.884511 & 0.274760 & 0.406274 & 0.043426 & 0.309307 & 0.130255 & nan & nan & 0.754832 & 0.231953 & nan & nan & 78 & 0.677277 & 0.033045 & 0.002859 & -6.458365 & 9.707849 & 336 & 0.519990 & 0.023400 & 0.003118 & -55.510678 & 3.817301 & 206 & 0.352012 & 0.038323 & 0.004204 & -86.102349 & 3.459306 \\
P2\_A & 214.869568 & 52.897374 & 227 & 0.501421 & 0.028585 & 0.003743 & -17.049038 & 3.590288 & 0.000368 & 0.000082 & 2.299040 & 0.946376 & 0.372037 & 0.085581 & 0.522566 & 0.258890 & nan & nan & 0.380347 & 0.127801 & nan & nan & 39 & 0.367035 & 0.071541 & 0.003892 & 4.715513 & 14.706015 & 188 & 0.652107 & 0.025441 & 0.004407 & -28.651152 & 4.845853 & 108 & 0.678300 & 0.032782 & 0.006022 & -70.772771 & 6.090818 \\
P2\_B & 214.920194 & 52.932849 & 187 & 0.372265 & 0.037800 & 0.003592 & -71.927794 & 2.856509 & 0.001025 & 0.000141 & 0.345772 & 0.068393 & 1.026255 & 0.257069 & 0.920663 & 0.509051 & nan & nan & 1.635251 & 1.806174 & nan & nan & 39 & 0.913313 & 0.023706 & 0.003869 & -53.343328 & 5.371234 & 148 & 0.376899 & 0.042897 & 0.004128 & -74.310252 & 3.100544 & 98 & 0.374554 & 0.053093 & 0.005211 & 83.782235 & 3.367598 \\
P2\_A1 & 214.851791 & 52.897374 & 46 & 0.264499 & 0.087475 & 0.008062 & -28.731696 & 2.855914 & 0.001536 & 0.000890 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 8 & 0.905843 & 0.049286 & 0.006237 & -52.667977 & 76.038445 & 38 & 0.261039 & 0.100329 & 0.009839 & -30.883092 & 3.116363 & 18 & 0.066604 & 0.225473 & 0.017019 & -52.025934 & 2.861978 \\
P2\_A2 & 214.869568 & 52.879596 & 52 & 0.433650 & 0.060460 & 0.005422 & 60.219006 & 2.664737 & 0.000808 & 0.000253 & nan & nan & 1.126186 & 0.617086 & nan & nan & nan & nan & nan & nan & nan & nan & 11 & 0.133057 & 0.201345 & 0.006996 & 37.522606 & 1.443993 & 41 & 0.585198 & 0.054776 & 0.005763 & 82.847748 & 3.936447 & 18 & 0.550373 & 0.078312 & 0.010913 & 30.761896 & 3.174309 \\
P2\_A3 & 214.869568 & 52.915151 & 65 & 0.684034 & 0.040569 & 0.007258 & 15.633288 & 6.857814 & 0.001408 & 0.000289 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 12 & 0.645506 & 0.086673 & 0.004795 & -17.520228 & 1.731268 & 53 & 0.698572 & 0.045158 & 0.008923 & 27.319057 & 4.871862 & 39 & 0.651184 & 0.058088 & 0.009005 & 71.232693 & 6.205285 \\
P2\_A4 & 214.887346 & 52.897374 & 61 & 0.253195 & 0.080617 & 0.009212 & -22.353815 & 2.417631 & 0.001370 & 0.000680 & 0.586259 & 0.228690 & 0.315974 & 0.030860 & 0.247160 & 0.101762 & nan & nan & nan & nan & nan & nan & 8 & 0.242152 & 0.187105 & 0.005576 & -25.022786 & 0.746649 & 53 & 0.480512 & 0.064919 & 0.009976 & -21.152670 & 3.284405 & 31 & 0.960110 & 0.020388 & 0.009908 & 66.582017 & 51.789972 \\
P2\_B1 & 214.937972 & 52.932849 & 56 & 0.109673 & 0.096514 & 0.005678 & -75.492862 & 1.493501 & 0.005281 & 0.000626 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 8 & 0.193847 & 0.155571 & 0.005898 & 64.265164 & 0.751098 & 48 & 0.099795 & 0.110946 & 0.007129 & -68.826467 & 1.455333 & 29 & 0.345656 & 0.096001 & 0.008039 & 85.215440 & 3.202490 \\
P2\_B2 & 214.920194 & 52.950627 & 44 & 0.450863 & 0.070877 & 0.008574 & 26.359909 & 4.265702 & 0.004847 & 0.000934 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 13 & 0.741448 & 0.077799 & 0.007902 & -26.844747 & 2.409779 & 31 & 0.252018 & 0.113059 & 0.011578 & 34.635201 & 3.569630 & 24 & 0.683211 & 0.065278 & 0.012717 & 60.380204 & 5.982565 \\
P2\_B3 & 214.920194 & 52.915071 & 44 & 0.143702 & 0.118873 & 0.008754 & -40.839651 & 1.751964 & 0.004906 & 0.000914 & 0.285948 & 0.045758 & 0.293200 & 0.034799 & 0.243609 & 0.048801 & nan & nan & nan & nan & nan & nan & 8 & 0.710272 & 0.130757 & 0.008844 & -29.263263 & 1.526934 & 36 & 0.187085 & 0.119849 & 0.009915 & -43.595084 & 2.155764 & 26 & 0.508450 & 0.094567 & 0.010117 & -67.259688 & 4.192903 \\
P2\_B4 & 214.902416 & 52.932849 & 43 & 0.279925 & 0.087456 & 0.005168 & 80.897709 & 2.262865 & 0.001004 & 0.000441 & 0.178645 & 0.018860 & 0.163738 & 0.017181 & 0.438629 & 0.172721 & nan & nan & 0.184429 & 0.053507 & nan & nan & 10 & 0.826576 & 0.065061 & 0.007184 & -83.557350 & 5.952334 & 33 & 0.314911 & 0.098005 & 0.006286 & 78.047263 & 2.438978 & 19 & 0.790791 & 0.058803 & 0.012796 & 40.623630 & 4.739732 \\
P3 & 214.803915 & 52.852283 & 389 & 0.086899 & 0.041343 & 0.002777 & 50.226748 & 1.792758 & 0.000528 & 0.000105 & 0.122015 & 0.048008 & 2.220713 & 1.709056 & 0.623325 & 0.080320 & nan & nan & 0.326335 & 0.067906 & 0.017343 & 0.015222 & 92 & 0.392533 & 0.045260 & 0.002580 & 13.753016 & 1.796900 & 297 & 0.066511 & 0.051788 & 0.003493 & 57.866120 & 1.785443 & 190 & 0.054613 & 0.067322 & 0.004915 & 58.363786 & 1.903937 \\
P3\_A & 214.777456 & 52.834881 & 192 & 0.113090 & 0.054433 & 0.003977 & 48.595439 & 1.810991 & 0.001208 & 0.000207 & 0.178559 & 0.062291 & 0.481082 & 0.173967 & 0.455606 & 0.124819 & nan & nan & 0.115600 & 0.031070 & nan & nan & 49 & 0.742844 & 0.034336 & 0.004031 & 47.245389 & 3.526908 & 143 & 0.152452 & 0.061211 & 0.005195 & 48.943507 & 2.031438 & 91 & 0.312658 & 0.060838 & 0.006770 & 45.016052 & 2.770433 \\
P3\_B & 214.830374 & 52.869685 & 197 & 0.562093 & 0.028790 & 0.003916 & 53.168736 & 3.713726 & 0.000335 & 0.000122 & 2.594834 & 7.361358 & 0.075265 & 0.048201 & 0.640213 & 0.112208 & nan & nan & 0.943701 & 0.210431 & 0.030923 & 0.022826 & 43 & 0.199032 & 0.089076 & 0.003793 & 8.408257 & 33.076976 & 154 & 0.298207 & 0.048801 & 0.005163 & 68.272436 & 2.659609 & 99 & 0.106851 & 0.082878 & 0.007058 & 67.220925 & 2.095598 \\
P3\_A1 & 214.759678 & 52.834881 & 52 & 0.819868 & 0.032550 & 0.007601 & 57.256273 & 4.908007 & 0.003596 & 0.000317 & 0.074224 & 0.019206 & 0.280469 & 0.274371 & 0.262861 & 0.084118 & nan & nan & nan & nan & nan & nan & 10 & 0.964711 & 0.029347 & 0.008255 & 58.094350 & 7.897804 & 42 & 0.848318 & 0.033670 & 0.008834 & 57.096358 & 6.425910 & 20 & 0.634563 & 0.075885 & 0.011580 & 41.313481 & 4.067263 \\
P3\_A2 & 214.777456 & 52.817104 & 43 & 0.985789 & 0.010249 & 0.005161 & -87.747385 & 63.235011 & 0.003584 & 0.000074 & nan & nan & nan & nan & nan & nan & nan & nan & 0.096267 & 0.058869 & nan & nan & 8 & 0.151869 & 0.244333 & 0.009391 & 6.348283 & 0.809338 & 35 & 0.748173 & 0.051727 & 0.007956 & -82.912794 & 5.757956 & 28 & 0.721604 & 0.063350 & 0.008675 & -72.446687 & 5.561905 \\
P3\_A3 & 214.777456 & 52.852659 & 48 & 0.016515 & 0.129214 & 0.005338 & 53.524593 & 1.370149 & 0.006611 & 0.000701 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 14 & 0.599474 & 0.071295 & 0.005115 & -84.836148 & 2.202652 & 34 & 0.005872 & 0.181716 & 0.007250 & 48.913594 & 1.226592 & 24 & 0.142385 & 0.140010 & 0.009660 & 43.441875 & 2.067579 \\
P3\_A4 & 214.795234 & 52.834881 & 49 & 0.482403 & 0.063797 & 0.010032 & 35.871172 & 3.930971 & 0.001858 & 0.000366 & 0.062943 & 0.027969 & 0.171914 & 0.046285 & 0.091478 & 0.026444 & nan & nan & 0.244076 & 0.216560 & nan & nan & 17 & 0.519870 & 0.088200 & 0.010444 & 64.385597 & 2.267259 & 32 & 0.512807 & 0.081245 & 0.013439 & 21.378072 & 4.733224 & 19 & 0.518273 & 0.106673 & 0.022597 & 29.077819 & 4.903119 \\
P3\_B1 & 214.848151 & 52.869685 & 50 & 0.294010 & 0.082430 & 0.008549 & 56.010766 & 2.873200 & 0.001802 & 0.000734 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 14 & 0.911398 & 0.035639 & 0.005112 & 52.274416 & 3.282438 & 36 & 0.310753 & 0.101195 & 0.011582 & 56.410442 & 3.311946 & 28 & 0.460252 & 0.093516 & 0.014226 & 61.814764 & 4.607998 \\
P3\_B2 & 214.830374 & 52.887463 & 51 & 0.536310 & 0.057892 & 0.007337 & 38.691899 & 69.653246 & 0.001206 & 0.000349 & 0.546098 & 0.060376 & 0.235119 & 0.075377 & 0.226673 & 0.070164 & nan & nan & 0.648205 & 0.549600 & 0.026962 & 0.014527 & 14 & 0.022283 & 0.270235 & 0.003932 & -4.750711 & 0.705154 & 37 & 0.852907 & 0.034214 & 0.010419 & 66.091526 & 8.403029 & 22 & 0.657753 & 0.074824 & 0.015701 & 88.989862 & 5.618478 \\
P3\_B3 & 214.830374 & 52.851907 & 49 & 0.135665 & 0.108768 & 0.006041 & -64.181405 & 2.304974 & 0.004471 & 0.000744 & 0.204882 & 0.082039 & 0.475950 & 0.282924 & 0.335270 & 0.116750 & nan & nan & nan & nan & nan & nan & 5 & 0.517757 & 0.142463 & 0.023142 & 28.119924 & 59.374112 & 44 & 0.077848 & 0.133173 & 0.006452 & -66.638362 & 2.033726 & 26 & 0.396205 & 0.101206 & 0.008247 & -73.183063 & 3.130010 \\
P3\_B4 & 214.812596 & 52.869685 & 47 & 0.115168 & 0.116048 & 0.006608 & 43.384931 & 2.132408 & 0.005831 & 0.000793 & 0.154507 & 0.026736 & 0.108226 & 0.030269 & 0.400877 & 0.074398 & nan & nan & 0.180361 & 0.022657 & nan & nan & 10 & 0.838073 & 0.059267 & 0.006235 & 73.398025 & 2.640083 & 37 & 0.103171 & 0.140606 & 0.008365 & 40.516396 & 2.211128 & 23 & 0.033212 & 0.221412 & 0.012105 & 47.878110 & 1.625014 \\
P4 & 214.757920 & 52.766983 & 372 & 0.042007 & 0.048136 & 0.003121 & 37.219571 & 1.831870 & 0.000880 & 0.000149 & 2.992551 & 5.094154 & 0.929310 & 0.230025 & 0.366322 & 0.085638 & nan & nan & 0.742248 & 0.593715 & 0.041015 & 0.043695 & 82 & 0.003723 & 0.113807 & 0.002880 & 29.297543 & 0.954052 & 290 & 0.370020 & 0.031773 & 0.004082 & 45.033029 & 3.273277 & 172 & 0.309240 & 0.046114 & 0.005554 & 65.060161 & 3.445045 \\
P4\_A & 214.783885 & 52.784217 & 186 & 0.266495 & 0.042204 & 0.004327 & 40.426064 & 2.942117 & 0.000783 & 0.000200 & 0.302818 & 0.069624 & 0.687220 & 0.343193 & 0.269403 & 0.077824 & nan & nan & nan & nan & 0.008994 & 0.005555 & 43 & 0.371169 & 0.067873 & 0.004610 & 29.647690 & 2.675512 & 143 & 0.477479 & 0.037180 & 0.005406 & 46.372884 & 4.117207 & 86 & 0.325690 & 0.062382 & 0.008039 & 50.298866 & 3.563072 \\
P4\_B & 214.731955 & 52.749748 & 186 & 0.154938 & 0.054276 & 0.004620 & 34.514178 & 2.199121 & 0.000726 & 0.000248 & 0.302617 & 0.055947 & 0.487963 & 0.095878 & 0.075082 & 0.038336 & nan & nan & 0.178087 & 0.053902 & 0.050196 & 0.050678 & 39 & 0.002797 & 0.165316 & 0.003321 & 29.101611 & 0.623615 & 147 & 0.700831 & 0.027899 & 0.005691 & 43.520924 & 5.291373 & 86 & 0.530500 & 0.049028 & 0.007133 & 84.702937 & 5.370001 \\
P4\_A1 & 214.801663 & 52.784217 & 50 & 0.797472 & 0.034352 & 0.009903 & 40.146613 & 6.995140 & 0.002221 & 0.000274 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 9 & 0.692665 & 0.116656 & 0.015186 & -71.697763 & 5.605947 & 41 & 0.523459 & 0.062619 & 0.011134 & 31.684995 & 4.092046 & 30 & 0.333111 & 0.096671 & 0.013612 & 58.924606 & 3.449146 \\
P4\_A2 & 214.783885 & 52.801995 & 42 & 0.384329 & 0.074767 & 0.007977 & -10.835065 & 2.478790 & 0.001466 & 0.000470 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 9 & 0.773558 & 0.076145 & 0.008070 & 18.689828 & 3.263043 & 33 & 0.390600 & 0.086579 & 0.009523 & -16.921154 & 2.624848 & 16 & 0.033590 & 0.250768 & 0.014053 & 5.685872 & 1.643778 \\
P4\_A3 & 214.783885 & 52.766440 & 50 & 0.100418 & 0.106571 & 0.010656 & 51.671626 & 2.367766 & 0.003566 & 0.001185 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 15 & 0.180959 & 0.127757 & 0.006938 & 42.911472 & 1.326302 & 35 & 0.291851 & 0.101981 & 0.015392 & 56.187034 & 3.832331 & 17 & 0.791209 & 0.073279 & 0.024482 & 61.845467 & 9.510263 \\
P4\_A4 & 214.766108 & 52.784217 & 44 & 0.648952 & 0.050041 & 0.006789 & 54.312342 & 4.909372 & 0.001884 & 0.000471 & 0.102420 & 0.013174 & 0.072020 & 0.015700 & 0.136108 & 0.035922 & nan & nan & nan & nan & nan & nan & 10 & 0.176167 & 0.181475 & 0.006420 & 12.601560 & 2.356243 & 34 & 0.458884 & 0.079247 & 0.010513 & 75.463953 & 2.963861 & 23 & 0.252087 & 0.132392 & 0.016185 & 81.327814 & 2.106477 \\
P4\_B1 & 214.714178 & 52.749748 & 50 & 0.603649 & 0.052148 & 0.008423 & 77.751805 & 5.108288 & 0.003036 & 0.000578 & 0.089727 & 0.008660 & 0.122528 & 0.027812 & 0.139720 & 0.046779 & nan & nan & 0.164686 & 0.060183 & nan & nan & 8 & 0.756289 & 0.077289 & 0.005817 & 30.994516 & 2.196139 & 42 & 0.552533 & 0.064090 & 0.009133 & 84.401738 & 5.035000 & 22 & 0.563464 & 0.083813 & 0.018906 & 68.276970 & 6.068756 \\
P4\_B2 & 214.731955 & 52.731971 & 40 & 0.018991 & 0.170361 & 0.005220 & 16.443546 & 1.020794 & 0.017493 & 0.000976 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 11 & 0.012225 & 0.244848 & 0.006932 & 30.290472 & 0.748934 & 29 & 0.125034 & 0.158182 & 0.006693 & 8.641071 & 1.489653 & 20 & 0.471297 & 0.123103 & 0.007176 & 7.529634 & 12.412034 \\
P4\_B3 & 214.731955 & 52.767526 & 46 & 0.234497 & 0.098623 & 0.006334 & 47.396246 & 2.102646 & 0.003455 & 0.000517 & 0.156700 & 0.010777 & nan & nan & 0.422084 & 0.143059 & nan & nan & nan & nan & nan & nan & 8 & 0.808458 & 0.083653 & 0.005852 & 60.699522 & 4.054743 & 38 & 0.285066 & 0.103742 & 0.007649 & 45.152221 & 2.278586 & 23 & 0.649975 & 0.077900 & 0.012003 & -86.857931 & 3.653676 \\
P4\_B4 & 214.749733 & 52.749748 & 50 & 0.949921 & 0.017796 & 0.008787 & 73.278293 & 66.691702 & 0.003147 & 0.000282 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 0.049015 & 0.140289 & 12 & 0.025749 & 0.244408 & 0.004462 & 21.856829 & 0.889800 & 38 & 0.615045 & 0.065752 & 0.014779 & -64.799693 & 6.215797 & 21 & 0.173564 & 0.165910 & 0.021671 & -83.023768 & 4.291385 \\
P5 & 214.941282 & 52.892913 & 326 & 0.869984 & 0.010700 & 0.002519 & -75.384052 & 7.679847 & 0.000609 & 0.000053 & 0.401933 & 0.065439 & 0.572757 & 0.140530 & 0.532092 & 0.155710 & nan & nan & 0.229154 & 0.046258 & 0.083380 & 0.126468 & 60 & 0.257861 & 0.063577 & 0.004673 & -59.141876 & 1.582456 & 266 & 0.937956 & 0.008340 & 0.002845 & 63.179563 & 13.367073 & 138 & 0.857936 & 0.018117 & 0.004748 & -22.000083 & 13.634149 \\
P5\_A & 214.968399 & 52.910539 & 161 & 0.115753 & 0.061376 & 0.003865 & -86.874627 & 2.049880 & 0.001398 & 0.000286 & 0.483852 & 0.087052 & 0.224939 & 0.055080 & 0.172545 & 0.097088 & nan & nan & 0.291984 & 0.075666 & 0.040674 & 0.036245 & 22 & 0.110302 & 0.128145 & 0.003594 & -86.406350 & 1.072614 & 139 & 0.301130 & 0.050945 & 0.004246 & -86.981956 & 2.754684 & 77 & 0.902876 & 0.020060 & 0.007336 & -66.870307 & 14.226270 \\
P5\_B & 214.914165 & 52.875287 & 165 & 0.318281 & 0.041891 & 0.003085 & -25.914433 & 59.193376 & 0.000715 & 0.000164 & 4.956747 & 2.655477 & 0.501199 & 0.089467 & 0.371263 & 0.150934 & nan & nan & 0.064307 & 0.019096 & 0.014258 & 0.005751 & 38 & 0.243722 & 0.083409 & 0.006900 & -35.637942 & 1.933833 & 127 & 0.316084 & 0.049772 & 0.003708 & 11.141653 & 2.105850 & 61 & 0.644922 & 0.045736 & 0.005797 & -14.352767 & 36.961613 \\
P5\_A1 & 214.986177 & 52.910539 & 39 & 0.860096 & 0.037862 & 0.009727 & 83.948841 & 82.015894 & 0.004344 & 0.000531 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 1 & 99.000000 & nan & nan & nan & nan & 38 & 0.906801 & 0.031170 & 0.010105 & -60.531703 & 73.598261 & 20 & 0.808261 & 0.063429 & 0.020357 & -29.906451 & 42.072818 \\
P5\_A2 & 214.968399 & 52.928317 & 26 & 0.374539 & 0.101397 & 0.007472 & -84.847489 & 2.458075 & 0.001076 & 0.000509 & 0.075266 & 0.018788 & 0.184855 & 0.031345 & 0.223084 & 0.041557 & nan & nan & nan & nan & nan & nan & 6 & 0.484400 & 0.168825 & 0.008947 & -71.273038 & 1.406216 & 20 & 0.569353 & 0.090630 & 0.009012 & 87.950266 & 3.599152 & 9 & 0.934133 & 0.044099 & 0.016023 & -33.627336 & 23.018279 \\
P5\_A3 & 214.968399 & 52.892762 & 45 & 0.495560 & 0.065033 & 0.006079 & 56.966127 & 3.299296 & 0.001503 & 0.000409 & nan & nan & nan & nan & nan & nan & nan & nan & 0.059599 & 0.020504 & nan & nan & 8 & 0.407686 & 0.099039 & 0.006464 & 84.458436 & 1.471458 & 37 & 0.568541 & 0.068917 & 0.008073 & 49.673836 & 3.527411 & 26 & 0.524876 & 0.086209 & 0.011491 & 37.109266 & 3.579440 \\
P5\_A4 & 214.950621 & 52.910539 & 51 & 0.003451 & 0.159338 & 0.005877 & -78.037367 & 1.122321 & 0.010583 & 0.000979 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 7 & 0.202052 & 0.224291 & 0.004749 & -86.665045 & 1.380283 & 44 & 0.013931 & 0.150601 & 0.006955 & -76.031877 & 1.348318 & 22 & 0.122222 & 0.160156 & 0.013171 & -70.747885 & 2.207009 \\
P5\_B1 & 214.896387 & 52.875287 & 35 & 0.709604 & 0.047620 & 0.005295 & 45.984476 & 3.194389 & 0.004582 & 0.000433 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 13 & 0.874226 & 0.050955 & 0.006854 & -64.572720 & 3.699505 & 22 & 0.379736 & 0.099756 & 0.007937 & 40.248685 & 1.939679 & 10 & 0.671858 & 0.103469 & 0.012718 & 19.229862 & 3.182134 \\
P5\_B2 & 214.914165 & 52.857509 & 35 & 0.213337 & 0.107457 & 0.006009 & -25.180763 & 2.394899 & 0.002404 & 0.000588 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 8 & 0.726765 & 0.077304 & 0.015336 & 11.912938 & 3.857855 & 27 & 0.195645 & 0.134455 & 0.007000 & -29.867078 & 2.249168 & 9 & 0.343856 & 0.211078 & 0.014154 & -38.532992 & 3.628194 \\
P5\_B3 & 214.914165 & 52.893064 & 56 & 0.470017 & 0.060569 & 0.005349 & -8.793976 & 24.993913 & 0.002908 & 0.000290 & 1.868284 & 1.981350 & 1.433190 & 1.333684 & 0.083016 & 0.035494 & nan & nan & 0.035503 & 0.008995 & nan & nan & 10 & 0.080094 & 0.187705 & 0.004712 & -27.294855 & 1.222838 & 46 & 0.647127 & 0.053302 & 0.005151 & 11.444210 & 6.439656 & 29 & 0.948136 & 0.023746 & 0.006140 & 29.747695 & 11.725260 \\
P5\_B4 & 214.931942 & 52.875287 & 39 & 0.734187 & 0.044389 & 0.007878 & 23.349320 & 4.699340 & 0.002518 & 0.000474 & 0.819899 & 0.131266 & 0.159553 & 0.032981 & 0.051211 & 0.022746 & nan & nan & 0.014534 & 0.004688 & 0.014761 & 0.007576 & 7 & 0.402723 & 0.175406 & 0.035852 & -50.359974 & 1.900052 & 32 & 0.379016 & 0.087754 & 0.008071 & 30.235368 & 2.023498 & 13 & 0.649681 & 0.089900 & 0.010915 & 56.993536 & 79.775451 \\
P6 & 214.856103 & 52.832955 & 374 & 0.261872 & 0.031902 & 0.002776 & 44.084031 & 2.259654 & 0.000285 & 0.000093 & 1.825314 & 0.835918 & 0.344830 & 0.053543 & 0.950281 & 0.517090 & nan & nan & 0.332768 & 0.144347 & 0.011452 & 0.011022 & 75 & 0.501960 & 0.043535 & 0.003570 & 39.957741 & 2.475942 & 299 & 0.431058 & 0.029256 & 0.003130 & 45.519031 & 3.111889 & 172 & 0.938032 & 0.010492 & 0.004011 & 46.737792 & 15.984769 \\
P6\_A & 214.830775 & 52.816234 & 189 & 0.135209 & 0.054355 & 0.003416 & 71.984302 & 1.767689 & 0.000984 & 0.000195 & 0.281948 & 0.066957 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 38 & 0.124650 & 0.098120 & 0.003905 & 64.417160 & 1.100578 & 151 & 0.373505 & 0.044726 & 0.004310 & 76.007863 & 2.554888 & 77 & 0.087937 & 0.094827 & 0.006300 & -74.585552 & 1.902343 \\
P6\_B & 214.881431 & 52.849675 & 185 & 0.124603 & 0.056990 & 0.004169 & 17.090651 & 2.161553 & 0.001103 & 0.000201 & 0.296921 & 0.113770 & nan & nan & nan & nan & nan & nan & 0.347797 & 0.159808 & 0.020935 & 0.018183 & 37 & 0.380249 & 0.078814 & 0.005517 & 22.049937 & 53.697785 & 148 & 0.232514 & 0.054605 & 0.005211 & 21.862742 & 2.488681 & 95 & 0.094014 & 0.086758 & 0.006219 & 20.456422 & 1.964050 \\
P6\_A1 & 214.812997 & 52.816234 & 35 & 0.722510 & 0.054155 & 0.006169 & 60.852720 & 2.979561 & 0.003080 & 0.000362 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 5 & 0.954502 & 0.056505 & 0.009586 & -62.352434 & 75.986661 & 30 & 0.639008 & 0.069675 & 0.006674 & 63.641020 & 2.464556 & 19 & 0.583965 & 0.091821 & 0.009745 & 77.968292 & 2.438915 \\
P6\_A2 & 214.830775 & 52.798457 & 51 & 0.509502 & 0.062580 & 0.007528 & 85.668452 & 2.830089 & 0.000963 & 0.000420 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 12 & 0.760171 & 0.058168 & 0.008108 & 62.119416 & 2.958497 & 39 & 0.558986 & 0.071850 & 0.010132 & -88.870863 & 3.202633 & 17 & 0.032511 & 0.261362 & 0.013870 & -77.766405 & 1.042553 \\
P6\_A3 & 214.830775 & 52.834012 & 60 & 0.353072 & 0.067340 & 0.006855 & 55.731385 & 2.742698 & 0.000584 & 0.000314 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 13 & 0.224864 & 0.146252 & 0.003700 & 57.514334 & 1.084292 & 47 & 0.705082 & 0.045972 & 0.008746 & 54.493090 & 5.535059 & 29 & 0.392422 & 0.090943 & 0.013290 & -43.453457 & 4.012344 \\
P6\_A4 & 214.848553 & 52.816234 & 43 & 0.535548 & 0.062348 & 0.005970 & 87.732161 & 2.867001 & 0.002809 & 0.000632 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 8 & 0.168575 & 0.194278 & 0.008791 & 77.738889 & 1.045819 & 35 & 0.836800 & 0.038537 & 0.006734 & -80.676196 & 5.807708 & 12 & 0.838178 & 0.064924 & 0.014489 & -89.828992 & 7.612323 \\
P6\_B1 & 214.899208 & 52.849675 & 29 & 0.618039 & 0.063578 & 0.007254 & -17.549474 & 3.915063 & 0.003202 & 0.000407 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 4 & 99.000000 & nan & nan & nan & nan & 25 & 0.819731 & 0.044870 & 0.009187 & -58.597941 & 78.817194 & 14 & 0.706557 & 0.075903 & 0.012699 & -15.173981 & 8.857384 \\
P6\_B2 & 214.881431 & 52.867453 & 32 & 0.261325 & 0.124230 & 0.013695 & 20.716672 & 3.580367 & 0.005298 & 0.001566 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 6 & 0.161436 & 0.325366 & 0.013807 & 13.531204 & 3.480276 & 26 & 0.619920 & 0.083344 & 0.017606 & 27.300940 & 5.308881 & 17 & 0.736711 & 0.085107 & 0.011889 & 37.782072 & 4.299791 \\
P6\_B3 & 214.881431 & 52.831897 & 57 & 0.330864 & 0.074112 & 0.008557 & 42.690892 & 2.535695 & 0.008313 & 0.000830 & 0.947771 & 0.238087 & 0.090296 & 0.033145 & 0.088467 & 0.021125 & nan & nan & 0.051226 & 0.022675 & nan & nan & 8 & 0.886371 & 0.068089 & 0.010478 & -22.580098 & 4.969490 & 49 & 0.215583 & 0.094168 & 0.009355 & 45.230312 & 2.396543 & 28 & 0.258069 & 0.119533 & 0.015177 & 47.234849 & 3.070997 \\
P6\_B4 & 214.863653 & 52.849675 & 67 & 0.437382 & 0.058750 & 0.006484 & 67.336233 & 85.004390 & 0.000835 & 0.000262 & nan & nan & nan & nan & nan & nan & nan & nan & 0.371985 & 0.082670 & nan & nan & 19 & 0.816852 & 0.045774 & 0.003600 & 31.848712 & 4.643641 & 48 & 0.424475 & 0.075041 & 0.008767 & -8.184421 & 21.902778 & 36 & 0.071108 & 0.148243 & 0.010017 & 6.369329 & 1.617576 \\
P7 & 215.107136 & 52.952446 & 380 & 0.103613 & 0.040310 & 0.002798 & -44.672987 & 1.937369 & 0.000591 & 0.000105 & 0.217633 & 0.028654 & 0.107852 & 0.052747 & 0.620705 & 0.089031 & nan & nan & 0.396446 & 0.325830 & 0.052856 & 0.053080 & 69 & 0.016477 & 0.108198 & 0.002304 & -51.194552 & 0.611204 & 311 & 0.475276 & 0.026298 & 0.003193 & -38.903208 & 3.565567 & 189 & 0.250230 & 0.046319 & 0.005293 & -35.459794 & 3.163307 \\
P7\_A & 215.132554 & 52.970139 & 198 & 0.037687 & 0.067979 & 0.003634 & -47.176954 & 1.547258 & 0.001874 & 0.000243 & 0.080442 & 0.018627 & 1.204591 & 0.749059 & 0.555798 & 0.112074 & nan & nan & 0.685963 & 0.887029 & 0.043535 & 0.020736 & 32 & 0.027620 & 0.151055 & 0.004207 & -56.757928 & 0.827617 & 166 & 0.186746 & 0.054563 & 0.004298 & -42.189683 & 2.221949 & 100 & 0.293736 & 0.060166 & 0.006197 & -42.841752 & 3.200453 \\
P7\_B & 215.081719 & 52.934754 & 182 & 0.900321 & 0.012350 & 0.003863 & -30.436438 & 19.248110 & 0.000884 & 0.000079 & 0.343277 & 0.050603 & 1.270409 & 0.402491 & 0.355616 & 0.058029 & nan & nan & 0.110104 & 0.026266 & 0.014685 & 0.018214 & 37 & 0.314200 & 0.077783 & 0.002655 & -41.756833 & 0.878751 & 145 & 0.945078 & 0.010483 & 0.004617 & 38.315723 & 37.446188 & 89 & 0.645986 & 0.037861 & 0.007127 & -21.265280 & 6.430805 \\
P7\_A1 & 215.150332 & 52.970139 & 47 & 0.164014 & 0.103065 & 0.008514 & -51.463128 & 2.697145 & 0.004561 & 0.000743 & 0.180194 & 0.031464 & nan & nan & nan & nan & nan & nan & 0.255737 & 0.244186 & nan & nan & 8 & 0.400910 & 0.165809 & 0.005955 & -67.137447 & 1.050738 & 39 & 0.287248 & 0.095967 & 0.010785 & -46.417548 & 3.144441 & 23 & 0.057064 & 0.202253 & 0.017042 & -48.215566 & 2.499493 \\
P7\_A2 & 215.132554 & 52.987917 & 58 & 0.013642 & 0.143449 & 0.005594 & -32.551358 & 1.165150 & 0.008506 & 0.000793 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 14 & 0.005197 & 0.233793 & 0.004724 & -41.910333 & 0.707598 & 44 & 0.132679 & 0.121216 & 0.007000 & -26.763495 & 1.786608 & 27 & 0.621789 & 0.074485 & 0.010238 & -20.553799 & 4.454905 \\
P7\_A3 & 215.132554 & 52.952361 & 55 & 0.863711 & 0.027720 & 0.007224 & -83.548278 & 8.563116 & 0.002303 & 0.000197 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 0.016450 & 0.008852 & 8 & 0.483235 & 0.171452 & 0.011195 & -76.027866 & 2.039274 & 47 & 0.970067 & 0.013571 & 0.006787 & 69.053793 & 34.382841 & 25 & 0.923082 & 0.030023 & 0.012914 & 57.614911 & 23.882146 \\
P7\_A4 & 215.114776 & 52.970139 & 38 & 0.633342 & 0.058149 & 0.007715 & -77.114680 & 3.363928 & 0.002174 & 0.000360 & 0.084998 & 0.027235 & 0.092470 & 0.034215 & 0.077336 & 0.020561 & nan & nan & 0.385128 & 0.408291 & nan & nan & 2 & 99.000000 & nan & nan & nan & nan & 36 & 0.608316 & 0.063376 & 0.007551 & -71.710777 & 3.219061 & 25 & 0.928273 & 0.028421 & 0.008632 & -57.386926 & 10.717856 \\
P7\_B1 & 215.063941 & 52.934754 & 44 & 0.827584 & 0.032355 & 0.007226 & 69.782538 & 9.086639 & 0.002334 & 0.000266 & 0.822223 & 0.300902 & 0.658375 & 0.086345 & 0.317235 & 0.077041 & nan & nan & nan & nan & nan & nan & 7 & 0.104180 & 0.156745 & 0.004401 & -56.081776 & 1.095564 & 37 & 0.667023 & 0.054629 & 0.010598 & 54.102000 & 5.440513 & 22 & 0.131987 & 0.157333 & 0.013141 & 82.822986 & 3.700983 \\
P7\_B2 & 215.081719 & 52.916976 & 41 & 0.751911 & 0.044207 & 0.008817 & -49.805621 & 4.125170 & 0.005452 & 0.000771 & 0.099608 & 0.012490 & 0.140759 & 0.021247 & 0.307640 & 0.097943 & nan & nan & 0.113208 & 0.049009 & nan & nan & 6 & 0.997175 & 0.012287 & 0.006447 & 74.768627 & 61.024095 & 35 & 0.714282 & 0.051949 & 0.009889 & -50.248362 & 4.056416 & 23 & 0.284088 & 0.123576 & 0.011180 & -31.453153 & 3.118184 \\
P7\_B3 & 215.081719 & 52.952531 & 44 & 0.977550 & 0.012016 & 0.005620 & -89.049965 & 71.615848 & 0.003810 & 0.000311 & 0.624970 & 0.165758 & 0.045319 & 0.012805 & 1.058224 & 5.864041 & nan & nan & nan & nan & nan & nan & 11 & 0.311829 & 0.155679 & 0.004923 & -18.019057 & 0.744436 & 33 & 0.809368 & 0.043676 & 0.008137 & 67.533409 & 6.870511 & 19 & 0.706903 & 0.081746 & 0.014425 & 64.164196 & 6.107217 \\
P7\_B4 & 215.099496 & 52.934754 & 53 & 0.690242 & 0.043234 & 0.008912 & -15.200769 & 22.352085 & 0.001652 & 0.000418 & nan & nan & 0.803678 & 0.696484 & 0.106816 & 0.022381 & nan & nan & 0.043682 & 0.008572 & nan & nan & 13 & 0.620481 & 0.083941 & 0.003065 & -64.321480 & 1.280825 & 40 & 0.522500 & 0.069147 & 0.011694 & -79.820421 & 85.565673 & 25 & 0.006670 & 0.228005 & 0.018076 & -9.301325 & 1.932273 \\
P8 & 215.014061 & 52.888246 & 421 & 0.033231 & 0.046751 & 0.002521 & -68.424518 & 1.523208 & 0.001378 & 0.000124 & 0.293263 & 0.075704 & 0.224808 & 0.091463 & 0.582851 & 0.273166 & nan & nan & 0.092902 & 0.023179 & 0.050838 & 0.027589 & 74 & 0.245222 & 0.062776 & 0.003859 & -70.678242 & 1.666149 & 347 & 0.100782 & 0.043363 & 0.002887 & -67.841984 & 1.910427 & 205 & 0.058476 & 0.061291 & 0.004162 & -65.584897 & 1.985684 \\
P8\_A & 215.040818 & 52.905737 & 198 & 0.018719 & 0.070448 & 0.003411 & -74.023257 & 1.319652 & 0.002999 & 0.000274 & 0.525053 & 0.171987 & 1.175476 & 0.707053 & 0.232139 & 0.101881 & nan & nan & 0.094869 & 0.024916 & 0.041287 & 0.039145 & 29 & 0.065540 & 0.106864 & 0.007992 & -67.932454 & 2.237043 & 169 & 0.071638 & 0.064851 & 0.003907 & -75.651184 & 1.616094 & 95 & 0.002420 & 0.129812 & 0.006265 & -71.026894 & 1.327361 \\
P8\_B & 214.987304 & 52.870755 & 223 & 0.514644 & 0.029446 & 0.003555 & -56.323999 & 3.297526 & 0.000631 & 0.000089 & 0.314082 & 0.035512 & 0.211535 & 0.028929 & 0.556493 & 0.600071 & nan & nan & nan & nan & nan & nan & 45 & 0.808612 & 0.035374 & 0.003791 & -76.062607 & 2.785660 & 178 & 0.563524 & 0.031002 & 0.004457 & -50.744597 & 3.884558 & 110 & 0.815237 & 0.022548 & 0.006268 & -26.918915 & 14.830814 \\
P8\_A1 & 215.058596 & 52.905737 & 50 & 0.159213 & 0.096763 & 0.005830 & 68.525197 & 1.781267 & 0.003686 & 0.000536 & 0.582989 & 0.262147 & 0.116090 & 0.016319 & 0.066374 & 0.039238 & nan & nan & 0.101630 & 0.042370 & nan & nan & 5 & 0.106094 & 0.302727 & 0.008684 & -52.556290 & 1.056046 & 45 & 0.061274 & 0.126613 & 0.005861 & 61.784315 & 1.512594 & 22 & 0.165020 & 0.135999 & 0.010736 & 65.306389 & 2.430936 \\
P8\_A2 & 215.040818 & 52.923514 & 38 & 0.037498 & 0.155123 & 0.007644 & -52.130251 & 1.616108 & 0.010205 & 0.001302 & nan & nan & nan & nan & nan & nan & nan & nan & 0.056436 & 0.019802 & nan & nan & 6 & 0.364786 & 0.167531 & 0.008886 & -54.119233 & 2.166464 & 32 & 0.084619 & 0.153237 & 0.009001 & -51.605036 & 1.886827 & 19 & 0.001286 & 0.322718 & 0.013450 & -50.268725 & 1.261353 \\
P8\_A3 & 215.040818 & 52.887959 & 66 & 0.322972 & 0.063876 & 0.006828 & -72.182963 & 2.632970 & 0.002181 & 0.000383 & 0.370834 & 0.075408 & nan & nan & 0.199174 & 0.040697 & nan & nan & 0.550391 & 0.582380 & 0.031238 & 0.022418 & 14 & 0.153081 & 0.110865 & 0.015312 & 81.484653 & 4.083927 & 52 & 0.430648 & 0.067127 & 0.008449 & -61.927553 & 2.720872 & 29 & 0.292626 & 0.104413 & 0.012544 & -85.612306 & 3.032879 \\
P8\_A4 & 215.023040 & 52.905737 & 44 & 0.169851 & 0.096803 & 0.006447 & -72.059271 & 2.346878 & 0.003306 & 0.000638 & 0.251403 & 0.067346 & 0.169638 & 0.041681 & 0.714341 & 0.915724 & nan & nan & 0.179315 & 0.031669 & nan & nan & 4 & 99.000000 & nan & nan & nan & nan & 40 & 0.181475 & 0.102810 & 0.007053 & -72.763524 & 2.331762 & 25 & 0.028710 & 0.200067 & 0.009722 & -68.947064 & 1.876140 \\
P8\_B1 & 214.969526 & 52.870755 & 63 & 0.294528 & 0.074854 & 0.004927 & 24.544834 & 57.553032 & 0.003508 & 0.000366 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 11 & 0.993755 & 0.013273 & 0.006562 & 41.582000 & 29.796700 & 52 & 0.236128 & 0.089389 & 0.005823 & 39.107824 & 71.395735 & 27 & 0.148136 & 0.126500 & 0.008039 & 12.893602 & 2.347787 \\
P8\_B2 & 214.987304 & 52.852977 & 56 & 0.154787 & 0.094637 & 0.007659 & -55.518421 & 2.519838 & 0.002405 & 0.000710 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 12 & 0.642977 & 0.101407 & 0.009646 & -72.471946 & 2.159440 & 44 & 0.204470 & 0.098564 & 0.009492 & -51.058303 & 2.929911 & 25 & 0.390351 & 0.102486 & 0.016378 & -56.002654 & 4.438601 \\
P8\_B3 & 214.987304 & 52.888533 & 58 & 0.403212 & 0.065938 & 0.005689 & -73.885591 & 2.007631 & 0.001748 & 0.000257 & 0.234064 & 0.037092 & 0.175936 & 0.063655 & 0.522079 & 0.155820 & nan & nan & 0.010185 & 0.006415 & nan & nan & 11 & 0.867436 & 0.059810 & 0.005893 & 76.072210 & 3.418638 & 47 & 0.383084 & 0.075737 & 0.006846 & -69.285634 & 2.114147 & 37 & 0.571608 & 0.066280 & 0.008311 & -89.283556 & 2.656160 \\
P8\_B4 & 215.005081 & 52.870755 & 46 & 0.742654 & 0.047139 & 0.009089 & 83.814504 & 6.666205 & 0.004821 & 0.000546 & 0.035165 & 0.019808 & 0.086048 & 0.045209 & 0.390731 & 0.155698 & nan & nan & nan & nan & nan & nan & 11 & 0.911683 & 0.044645 & 0.005250 & -39.335527 & 4.954276 & 35 & 0.654097 & 0.067905 & 0.011633 & 78.326840 & 5.768507 & 21 & 0.502538 & 0.100832 & 0.017557 & -16.364172 & 22.936304 \\
P9 & 214.920408 & 52.825661 & 371 & 0.964801 & 0.005251 & 0.002290 & 85.265820 & 17.141299 & 0.000390 & 0.000016 & 4.178060 & 4.121620 & 0.111237 & 0.053887 & 0.290828 & 0.094227 & nan & nan & 0.393928 & 0.181731 & 0.014512 & 0.007105 & 72 & 0.306482 & 0.059923 & 0.002264 & -6.853429 & 1.111149 & 299 & 0.656372 & 0.020615 & 0.003196 & 83.796210 & 3.812425 & 152 & 0.515322 & 0.036545 & 0.004915 & 70.151297 & 3.557954 \\
P9\_A & 214.947317 & 52.843592 & 157 & 0.718914 & 0.024284 & 0.003887 & 66.182081 & 83.328935 & 0.000629 & 0.000089 & 0.214955 & 0.046287 & 0.038039 & 0.020376 & 0.083036 & 0.062279 & nan & nan & 0.514637 & 0.405837 & nan & nan & 35 & 0.153225 & 0.099612 & 0.003597 & 69.605437 & 86.773900 & 122 & 0.985125 & 0.006142 & 0.003124 & 77.511543 & 59.918210 & 60 & 0.608077 & 0.050339 & 0.006318 & 53.116016 & 4.936090 \\
P9\_B & 214.893499 & 52.807730 & 214 & 0.607388 & 0.025991 & 0.003452 & 89.547088 & 3.576625 & 0.000587 & 0.000104 & 0.054911 & 0.028114 & 0.052816 & 0.030219 & 2.461222 & 2.180991 & nan & nan & 0.043143 & 0.017019 & 0.012141 & 0.008018 & 37 & 0.843314 & 0.034236 & 0.003132 & -28.360727 & 2.185664 & 177 & 0.464450 & 0.035964 & 0.004063 & 84.792075 & 2.864076 & 92 & 0.658171 & 0.037560 & 0.006164 & 84.452303 & 4.383531 \\
P9\_A1 & 214.965094 & 52.843592 & 37 & 0.723984 & 0.051061 & 0.007078 & -49.722938 & 5.016293 & 0.004736 & 0.000672 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 7 & 0.311376 & 0.191601 & 0.006570 & 4.793178 & 1.021817 & 30 & 0.485089 & 0.087585 & 0.009156 & -63.929166 & 3.348925 & 13 & 0.958994 & 0.032955 & 0.016153 & -80.077717 & 24.959749 \\
P9\_A2 & 214.947317 & 52.861370 & 35 & 0.832028 & 0.039465 & 0.006849 & -30.476034 & 5.654807 & 0.003484 & 0.000264 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 8 & 0.054868 & 0.318997 & 0.005691 & -29.441538 & 1.035007 & 27 & 0.829950 & 0.045266 & 0.008549 & 61.499344 & 6.067626 & 17 & 0.871638 & 0.043910 & 0.009132 & -38.024489 & 7.491338 \\
P9\_A3 & 214.947317 & 52.825814 & 49 & 0.840037 & 0.029894 & 0.005692 & 80.155031 & 5.230892 & 0.002179 & 0.000154 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 12 & 0.270736 & 0.116345 & 0.006263 & 24.811918 & 1.407280 & 37 & 0.596681 & 0.063778 & 0.007752 & -82.923813 & 2.821405 & 21 & 0.398265 & 0.120265 & 0.008822 & 49.463875 & 2.515312 \\
P9\_A4 & 214.929539 & 52.843592 & 36 & 0.056984 & 0.152323 & 0.008673 & 15.034683 & 1.672855 & 0.008333 & 0.001106 & 0.107224 & 0.035624 & 0.098185 & 0.053969 & 0.015805 & 0.010151 & nan & nan & 0.158713 & 0.055348 & nan & nan & 8 & 0.518735 & 0.117871 & 0.006907 & 46.533577 & 1.563162 & 28 & 0.057896 & 0.183466 & 0.011806 & 10.260572 & 1.620604 & 9 & 0.627242 & 0.141483 & 0.022827 & 52.499852 & 7.730623 \\
P9\_B1 & 214.875721 & 52.807730 & 53 & 0.495967 & 0.064570 & 0.007670 & -67.729181 & 3.207329 & 0.005420 & 0.000507 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 6 & 0.367826 & 0.214047 & 0.006245 & -60.320163 & 1.597483 & 47 & 0.724552 & 0.047084 & 0.008697 & -71.730312 & 5.024093 & 28 & 0.639214 & 0.070055 & 0.010452 & -37.806853 & 4.686675 \\
P9\_B2 & 214.893499 & 52.789952 & 70 & 0.419696 & 0.055937 & 0.005296 & -52.646507 & 2.372000 & 0.000731 & 0.000279 & 0.165636 & 0.050945 & 0.092491 & 0.046321 & 0.203340 & 0.078577 & nan & nan & 0.173722 & 0.069801 & nan & nan & 11 & 0.036060 & 0.208959 & 0.004365 & -38.683300 & 0.680286 & 59 & 0.741962 & 0.037053 & 0.006271 & -67.647652 & 4.329674 & 27 & 0.925342 & 0.028260 & 0.007835 & -48.072927 & 8.270279 \\
P9\_B3 & 214.893499 & 52.825508 & 42 & 0.459752 & 0.069127 & 0.006167 & -84.197052 & 2.473673 & 0.000952 & 0.000328 & 0.211167 & 0.047823 & 0.066604 & 0.029382 & 0.239015 & 0.040619 & nan & nan & nan & nan & nan & nan & 12 & 0.590519 & 0.101961 & 0.004206 & -89.665696 & 1.463232 & 30 & 0.697799 & 0.057136 & 0.008548 & -79.881705 & 4.178348 & 17 & 0.569173 & 0.097203 & 0.012893 & -84.389927 & 3.756932 \\
P9\_B4 & 214.911277 & 52.807730 & 49 & 0.061513 & 0.140335 & 0.006512 & 41.825058 & 1.687195 & 0.010085 & 0.001077 & 1.052161 & 0.297015 & 0.134037 & 0.019939 & nan & nan & nan & nan & 0.016300 & 0.007159 & nan & nan & 8 & 0.044994 & 0.386712 & 0.005223 & 24.079702 & 0.582758 & 41 & 0.203670 & 0.114764 & 0.007697 & 53.089861 & 2.432248 & 20 & 0.103606 & 0.210267 & 0.014655 & 60.714698 & 2.334251 \\
P10 & 214.828677 & 52.763124 & 349 & 0.098892 & 0.043225 & 0.003818 & -38.084015 & 2.305315 & 0.000557 & 0.000155 & 0.557266 & 0.105303 & 0.929178 & 0.462795 & 1.305308 & 0.784671 & nan & nan & 0.767243 & 1.005225 & 0.038597 & 0.054087 & 66 & 0.708254 & 0.030025 & 0.002407 & -50.414758 & 2.761029 & 283 & 0.131050 & 0.047028 & 0.004538 & -36.398225 & 2.619984 & 174 & 0.076875 & 0.067761 & 0.005897 & -19.102458 & 2.780235 \\
P10\_A & 214.855572 & 52.781364 & 195 & 0.469446 & 0.033673 & 0.005129 & -44.061159 & 4.059617 & 0.000612 & 0.000167 & 0.379006 & 0.085772 & 1.302063 & 1.871101 & 0.300860 & 0.052553 & nan & nan & 0.252999 & 0.306981 & 0.072692 & 0.098955 & 37 & 0.792193 & 0.036565 & 0.003271 & -74.333400 & 2.787983 & 158 & 0.479344 & 0.038099 & 0.006554 & -38.294982 & 4.345668 & 89 & 0.491853 & 0.050376 & 0.007353 & 55.655964 & 78.105684 \\
P10\_B & 214.801782 & 52.744885 & 154 & 0.153226 & 0.057290 & 0.005091 & -33.862367 & 2.647931 & 0.000957 & 0.000255 & 0.945722 & 0.194329 & 0.372077 & 0.107508 & nan & nan & nan & nan & nan & nan & nan & nan & 29 & 0.553991 & 0.050535 & 0.004042 & -29.105196 & 2.390747 & 125 & 0.240820 & 0.058918 & 0.006089 & -34.805811 & 3.212114 & 85 & 0.037398 & 0.108596 & 0.008519 & -28.770731 & 2.487636 \\
P10\_A1 & 214.873350 & 52.781364 & 53 & 0.851170 & 0.030539 & 0.006567 & -29.581897 & 50.733660 & 0.002733 & 0.000265 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 6 & 0.579246 & 0.119018 & 0.006378 & -58.646294 & 2.079479 & 47 & 0.806071 & 0.038969 & 0.008343 & 81.063046 & 83.818434 & 20 & 0.418732 & 0.114464 & 0.015075 & 55.493208 & 4.126619 \\
P10\_A2 & 214.855572 & 52.799142 & 44 & 0.328280 & 0.084051 & 0.010921 & -69.377105 & 4.247449 & 0.008700 & 0.001138 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 10 & 0.407698 & 0.136198 & 0.006950 & 73.008921 & 1.194565 & 34 & 0.291705 & 0.104807 & 0.015657 & -58.623404 & 4.156406 & 18 & 0.579581 & 0.102565 & 0.011055 & -44.159727 & 3.267581 \\
P10\_A3 & 214.855572 & 52.763586 & 53 & 0.684505 & 0.043652 & 0.007804 & -36.406165 & 6.267493 & 0.003194 & 0.000474 & 0.073653 & 0.017745 & 0.871605 & 0.861963 & 0.269975 & 0.051576 & nan & nan & 0.199267 & 0.243929 & 0.015516 & 0.032449 & 16 & 0.959494 & 0.023017 & 0.005553 & 18.020953 & 14.219834 & 37 & 0.589318 & 0.065091 & 0.010770 & -40.324949 & 5.898274 & 25 & 0.303549 & 0.116774 & 0.017909 & 9.848378 & 20.382312 \\
P10\_A4 & 214.837794 & 52.781364 & 45 & 0.821489 & 0.037998 & 0.012761 & -31.759054 & 19.257125 & 0.003251 & 0.000699 & nan & nan & nan & nan & nan & nan & nan & nan & 0.121370 & 0.048697 & nan & nan & 5 & 0.604934 & 0.206220 & 0.009196 & -44.609275 & 1.078353 & 40 & 0.909178 & 0.027768 & 0.011384 & -57.068985 & 65.203735 & 26 & 0.531695 & 0.093008 & 0.016278 & -36.846773 & 62.525016 \\
P10\_B1 & 214.784004 & 52.744885 & 28 & 0.309064 & 0.089245 & 0.008455 & -25.054384 & 3.080915 & 0.003347 & 0.000719 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 9 & 0.983425 & 0.009904 & 0.004019 & 35.232193 & 37.933146 & 19 & 0.272939 & 0.132437 & 0.013146 & -26.065588 & 2.884392 & 13 & 0.305155 & 0.140870 & 0.018774 & -31.647299 & 3.584153 \\
P10\_B2 & 214.801782 & 52.727107 & 53 & 0.359012 & 0.076387 & 0.010376 & -26.269793 & 3.204314 & 0.000931 & 0.000498 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 6 & 0.682478 & 0.119297 & 0.009824 & -40.274156 & 3.220785 & 47 & 0.456013 & 0.072895 & 0.011608 & -23.619696 & 3.808947 & 34 & 0.315417 & 0.108396 & 0.016573 & -14.119642 & 3.428645 \\
P10\_B3 & 214.801782 & 52.762663 & 31 & 0.677563 & 0.062644 & 0.014606 & -39.484449 & 7.024546 & 0.007802 & 0.001000 & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & nan & 6 & 0.083727 & 0.250870 & 0.007306 & -37.731073 & 1.032324 & 25 & 0.947498 & 0.027603 & 0.015871 & -69.155304 & 43.611492 & 16 & 0.367614 & 0.143396 & 0.030404 & -43.529212 & 5.340915 \\
P10\_B4 & 214.819560 & 52.744885 & 42 & 0.803686 & 0.036948 & 0.007814 & -65.737985 & 5.949433 & 0.003689 & 0.000401 & 0.210008 & 0.044824 & 0.810862 & 0.335719 & nan & nan & nan & nan & nan & nan & nan & nan & 8 & 0.504866 & 0.112301 & 0.006383 & 37.971188 & 2.817155 & 34 & 0.570204 & 0.069583 & 0.009304 & -60.803011 & 4.123734 & 22 & 0.441421 & 0.105369 & 0.009639 & -35.183096 & 4.705622 \\
\end{tabular}
\end{table}

